Retrieval-style In-Context Learning for Few-shot Hierarchical Text Classification

Hierarchical text classification (HTC) is an important task with broad applications, while few-shot HTC has gained increasing interest recently. While in-context learning (ICL) with large language models (LLMs) has achieved significant success in few-shot learning, it is not as effective for HTC because of the expansive hierarchical label sets and extremely-ambiguous labels. In this work, we introduce the first ICL-based framework with LLM for few-shot HTC. We exploit a retrieval database to identify relevant demonstrations, and an iterative policy to manage multi-layer hierarchical labels. Particularly, we equip the retrieval database with HTC label-aware representations for the input texts, which is achieved by continual training on a pretrained language model with masked language modeling (MLM), layer-wise classification (CLS, specifically for HTC), and a novel divergent contrastive learning (DCL, mainly for adjacent semantically-similar labels) objective. Experimental results on three benchmark datasets demonstrate superior performance of our method, and we can achieve state-of-the-art results in few-shot HTC.

==> tables/main_result.tex <==
\begin{table*}[!htbp]
    \centering
    % \normalsize
    % \addtolength{\tabcolsep}{-3pt}
    \resizebox{2\columnwidth}{!}{
        \begin{tabular}{c l c c c c c c}
            \toprule
            
            \multirow{2}{*}{Q} & \makecell[c]{\multirow{2}{*}{Method}} & \multicolumn{2}{c}{\textbf{WOS(Depth 2)}} & \multicolumn{2}{c}{\textbf{DBpedia(Depth 3)}} & \multicolumn{2}{c}{\textbf{Patent(Depth 4)}} \\ \cmidrule{3-8}
                               &                                       &       Micro-F1      &       Macro-F1      &       Micro-F1       &        Macro-F1        &       Micro-F1      &        Macro-F1        \\ \midrule
            
            \multirow{9}{*}{1} &              BERT (Vanilla FT)                     &           2.99  $\pm$ 20.85 {\color{olivegreen}(5.12)} &           0.16  $\pm$ 0.10 {\color{olivegreen}(0.24)}  &           14.43  $\pm$ 13.34 {\color{olivegreen}(24.27)} &           0.29  $\pm$ 0.01 {\color{olivegreen}(0.32)}  &           27.04  $\pm$ 1.48  {\color{olivegreen}(28.37)} &           2.40  $\pm$ 0.23 {\color{olivegreen}(2.67)}   \\
                               & Llama-7B (Vanilla FT) & 35.19 & 30.39 & & & & \\
                               &  HiMatch \cite{chen-etal-2021-hierarchy}           &           43.44 $\pm$ 8.09 {\color{olivegreen}(48.26)} &           7.71  $\pm$ 4.90 {\color{olivegreen}(9.32)}  &                                 -                        &                               -                        &                               -                          &                             -                           \\
                               &  HGCLR   \cite{wang-etal-2022-incorporating}       &           9.77  $\pm$ 11.77 {\color{olivegreen}(16.32)}&           0.59  $\pm$ 0.10 {\color{olivegreen}(0.63)}  &           15.73  $\pm$ 31.07 {\color{olivegreen}(25.13)} &           0.28  $\pm$ 0.10 {\color{olivegreen}(0.31)}  &           28.99  $\pm$ 1.12  {\color{olivegreen}(29.89)} &           2.94  $\pm$ 0.24 {\color{olivegreen}(3.13)}   \\
                               &  HPT     \cite{wang-etal-2022-hpt}                 &           50.05 $\pm$ 6.80 {\color{olivegreen}(50.96)} &           25.69 $\pm$ 3.31 {\color{olivegreen}(27.76)} &           72.52  $\pm$ 10.20 {\color{olivegreen}(73.47)} &           31.01 $\pm$ 2.61 {\color{olivegreen}(32.50)} &           35.22  $\pm$ 1.07  {\color{olivegreen}(36.26)} &           4.22  $\pm$ 0.68 {\color{olivegreen}(4.87)}   \\
                               &  HierVerb \cite{ji-etal-2023-hierarchical} &           58.95 $\pm$ 6.38 {\color{olivegreen}(61.76)} &           44.96 $\pm$ 4.86 {\color{olivegreen}(48.19)} &           91.81  $\pm$ 0.07  {\color{olivegreen}(91.95)} &           85.32 $\pm$ 0.04 {\color{olivegreen}(85.44)} &           41.83  $\pm$ 0.60  {\color{olivegreen}(42.52)} &           5.91  $\pm$ 0.65 {\color{olivegreen}(6.53)}   \\
                               \cmidrule{2-8}
                               &                    Ours Retrieval (Top1)                     &\underline{63.46}$\pm$ 2.30 {\color{olivegreen}(65.99)} &\underline{50.24}$\pm$ 2.21 {\color{olivegreen}(52.66)} &\underline{93.68} $\pm$ 0.05  {\color{olivegreen}(93.74)} &\underline{88.41}$\pm$ 0.23 {\color{olivegreen}(88.67)} &\underline{47.71} $\pm$ 0.41  {\color{olivegreen}(48.15)} &\underline{10.76}$\pm$ 0.25 {\color{olivegreen}(11.02)}  \\
                               & Ours Llama-7B (Top3) + ICL & 65.61 & 36.50 & 92.44 & 85.70 & & \\
                               &                 Ours ChatGPT (Top3) + ICL                  &\textbf{   68.91 $\pm$ 0.48 {\color{olivegreen}(69.38)}}&\textbf{   57.41 $\pm$ 0.40 {\color{olivegreen}(57.82)}}&\textbf{   94.54  $\pm$ 0.03  {\color{olivegreen}(94.58)}}&\textbf{   89.75 $\pm$ 0.09 {\color{olivegreen}(94.83)}}&\textbf{   52.23  $\pm$ 0.23  {\color{olivegreen}(52.45)}}&\textbf{   15.62 $\pm$ 0.17 {\color{olivegreen}(15.78)}} \\  \midrule

            \multirow{9}{*}{2} &              BERT (Vanilla FT)                     &           46.31  $\pm$ 0.65 {\color{olivegreen}(46.85)} &           5.11  $\pm$ 1.31 {\color{olivegreen}(5.51)}  &           87.02  $\pm$ 3.89  {\color{olivegreen}(88.20)} &           69.05 $\pm$ 26.81{\color{olivegreen}(73.28)} &           36.07  $\pm$ 0.24  {\color{olivegreen}(36.88)} &           6.41  $\pm$ 0.77 {\color{olivegreen}(6.92)}   \\
                               & Llama-7B (Vanilla FT) & 49.02 & 40.97 & & & & \\
                               &  HiMatch \cite{chen-etal-2021-hierarchy}           &           46.41  $\pm$ 1.31 {\color{olivegreen}(47.23)} &           18.97 $\pm$ 0.65 {\color{olivegreen}(21.06)} &                                 -                        &                               -                        &                               -                          &                             -                           \\
                               &  HGCLR   \cite{wang-etal-2022-incorporating}       &           45.11  $\pm$ 5.02 {\color{olivegreen}(47.56)} &           5.80  $\pm$ 11.63{\color{olivegreen}(9.63)}  &           87.79  $\pm$ 0.40  {\color{olivegreen}(88.42)} &           71.46 $\pm$ 0.17 {\color{olivegreen}(71.78)} &           36.73  $\pm$ 1.13  {\color{olivegreen}(38.03)} &           6.82  $\pm$ 0.21 {\color{olivegreen}(7.06)}   \\
                               &  HPT     \cite{wang-etal-2022-hpt}                 &           57.45  $\pm$ 1.89 {\color{olivegreen}(58.99)} &           35.97 $\pm$ 11.89{\color{olivegreen}(39.94)} &           90.32  $\pm$ 0.64  {\color{olivegreen}(91.11)} &           81.12 $\pm$ 1.33 {\color{olivegreen}(82.42)} &           42.61  $\pm$ 0.75  {\color{olivegreen}(43.43)} &           10.53 $\pm$ 0.30 {\color{olivegreen}(10.87)}  \\
                               &  HierVerb \cite{ji-etal-2023-hierarchical} &           66.08  $\pm$ 4.19 {\color{olivegreen}(68.01)} &           54.04 $\pm$ 3.24 {\color{olivegreen}(56.69)} &           93.71  $\pm$ 0.01  {\color{olivegreen}(93.87)} &           88.96 $\pm$ 0.02 {\color{olivegreen}(89.02)} &           48.42  $\pm$ 0.39  {\color{olivegreen}(48.74)} &           12.97 $\pm$ 0.39 {\color{olivegreen}(13.24)}  \\  \cmidrule{2-8}
                               &                    Ours (Top1)                     &\underline{69.85} $\pm$ 0.63 {\color{olivegreen}(70.58)} &\underline{58.64}$\pm$ 0.58 {\color{olivegreen}(59.25)} &\underline{94.12} $\pm$ 0.18  {\color{olivegreen}(94.32)} &\underline{89.33}$\pm$ 0.19 {\color{olivegreen}(89.54)} &\underline{51.63} $\pm$ 0.34  {\color{olivegreen}(51.91)} &\underline{15.12}$\pm$ 0.23 {\color{olivegreen}(15.32)}  \\  
                               & Llama + ICL & 67.09 & 54.70 &  & & & \\
                               &                 Ours (Top3) + ICL                  &\textbf{   71.68  $\pm$ 0.09 {\color{olivegreen}(71.76)}}&\textbf{   61.99 $\pm$ 0.10 {\color{olivegreen}(62.08)}}&\textbf{   94.87  $\pm$ 0.10  {\color{olivegreen}(94.97)}}&\textbf{   90.82 $\pm$ 0.08 {\color{olivegreen}(90.89)}}&\textbf{   56.84  $\pm$ 0.11  {\color{olivegreen}(56.93)}}&\textbf{   20.07 $\pm$ 0.10 {\color{olivegreen}(20.17)}} \\  \midrule
            
            \multirow{8}{*}{4} &              BERT (Vanilla FT)                     &           56.00  $\pm$ 4.25 {\color{olivegreen}(57.18)} &           31.04 $\pm$ 16.65{\color{olivegreen}(33.77)} &           92.94  $\pm$ 0.66  {\color{olivegreen}(93.38)} &           84.63 $\pm$ 0.17 {\color{olivegreen}(85.47)} &           49.41 $\pm$ 0.98 {\color{olivegreen}(50.24)} &           9.64  $\pm$ 0.56 {\color{olivegreen}(10.13)} \\
                               &  HiMatch \cite{chen-etal-2021-hierarchy}           &           57.43  $\pm$ 0.01 {\color{olivegreen}(57.43)} &           39.04 $\pm$ 0.01 {\color{olivegreen}(39.04)} &                                -                         &                               -                        &                               -                        &                             -                          \\
                               &  HGCLR   \cite{wang-etal-2022-incorporating}       &           56.80  $\pm$ 4.24 {\color{olivegreen}(57.96)} &           32.34 $\pm$ 15.39{\color{olivegreen}(33.76)} &           93.14  $\pm$ 0.01  {\color{olivegreen}(93.22)} &           84.74 $\pm$ 0.11 {\color{olivegreen}(85.11)} &           50.24 $\pm$ 0.36 {\color{olivegreen}(50.63)} &           11.40 $\pm$ 0.29 {\color{olivegreen}(11.67)} \\
                               &  HPT     \cite{wang-etal-2022-hpt}                 &           65.57  $\pm$ 1.69 {\color{olivegreen}(67.06)} &           45.89 $\pm$ 9.78 {\color{olivegreen}(49.42)} &           94.34  $\pm$ 0.28  {\color{olivegreen}(94.83)} &           90.09 $\pm$ 0.87 {\color{olivegreen}(91.12)} &           53.91 $\pm$ 0.44 {\color{olivegreen}(54.29)} &           18.45 $\pm$ 0.40 {\color{olivegreen}(18.79)} \\
                               &  HierVerb \cite{ji-etal-2023-hierarchical} &           72.58  $\pm$ 0.83 {\color{olivegreen}(73.64)} &           63.12 $\pm$ 1.48 {\color{olivegreen}(64.47)} &           94.75  $\pm$ 0.13  {\color{olivegreen}(95.13)} &           90.77 $\pm$ 0.33 {\color{olivegreen}(91.43)} &           58.17 $\pm$ 0.41 {\color{olivegreen}(58.64)} &           23.28 $\pm$ 0.39 {\color{olivegreen}(23.63)} \\  \cmidrule{2-8}
                               &                    Ours (Top1)                     &\underline{75.37} $\pm$ 0.70 {\color{olivegreen}(76.08)} &\underline{65.94}$\pm$ 0.57 {\color{olivegreen}(66.41)} &\underline{95.15} $\pm$ 0.07  {\color{olivegreen}(95.23)} &\underline{91.26}$\pm$ 0.14 {\color{olivegreen}(91.38)} &\textbf{   60.53 $\pm$ 0.36 {\color{olivegreen}(60.82)}}&\textbf{   25.65 $\pm$ 0.29 {\color{olivegreen}(25.95)}}\\  
                               & Llama + ICL & 71.68 & 60.22 &  & & & \\
                               &                 Ours (Top3) + ICL                  &\textbf{   75.62  $\pm$ 0.15 {\color{olivegreen}(75.78)}}&\textbf{   66.34 $\pm$ 0.09 {\color{olivegreen}(66.41)}}&\textbf{   95.26  $\pm$ 0.07  {\color{olivegreen}(95.23)}}&\textbf{   91.42 $\pm$ 0.05 {\color{olivegreen}(91.47)}}&\underline{59.35}$\pm$ 0.10 {\color{olivegreen}(59.45)} &\underline{24.15}$\pm$ 0.08 {\color{olivegreen}(24.25)} \\  \midrule

            \multirow{8}{*}{8} &              BERT (Vanilla FT)                     &           66.24  $\pm$ 1.96 {\color{olivegreen}(67.53)} &           50.21 $\pm$ 5.05 {\color{olivegreen}(52.60)} &           94.39  $\pm$ 0.06  {\color{olivegreen}(94.57)} &           87.63 $\pm$ 0.28 {\color{olivegreen}(87.78)} &           62.10  $\pm$ 1.34 {\color{olivegreen}(63.29)}  &           26.85 $\pm$ 0.97 {\color{olivegreen}(27.75)}  \\
                               &  HiMatch \cite{chen-etal-2021-hierarchy}           &           69.92  $\pm$ 0.01 {\color{olivegreen}(70.23)} &           57.47 $\pm$ 0.01 {\color{olivegreen}(57.78)} &                                 -                        &                               -                        &                               -                          &                             -                           \\
                               &  HGCLR   \cite{wang-etal-2022-incorporating}       &           68.34  $\pm$ 0.96 {\color{olivegreen}(69.22)} &           54.41 $\pm$ 2.97 {\color{olivegreen}(55.99)} &           94.70  $\pm$ 0.05  {\color{olivegreen}(94.94)} &           88.04 $\pm$ 0.25 {\color{olivegreen}(88.61)} &           64.69  $\pm$ 0.30 {\color{olivegreen}(65.01)}  &           27.69 $\pm$ 0.47 {\color{olivegreen}(28.21)}  \\
                               &  HPT     \cite{wang-etal-2022-hpt}                 &           76.22  $\pm$ 0.99 {\color{olivegreen}(77.23)} &           67.20 $\pm$ 1.89 {\color{olivegreen}(68.63)} &           95.49  $\pm$ 0.01  {\color{olivegreen}(95.57)} &           92.35 $\pm$ 0.03 {\color{olivegreen}(92.52)} &           67.35  $\pm$ 0.13 {\color{olivegreen}(67.45)}  &           28.39 $\pm$ 0.08 {\color{olivegreen}(28.46)}  \\
                               &  HierVerb \cite{ji-etal-2023-hierarchical} &\underline{78.12} $\pm$ 0.55 {\color{olivegreen}(78.87)} &\underline{69.98}$\pm$ 0.91 {\color{olivegreen}(71.04)} &\underline{95.69} $\pm$ 0.01  {\color{olivegreen}(95.70)} &\underline{92.44 $\pm$ 0.01 {\color{olivegreen}(92.51)}}&\underline{68.74} $\pm$ 0.12 {\color{olivegreen}(68.82)}  &\underline{29.93}$\pm$ 0.07 {\color{olivegreen}(30.01)}  \\  \cmidrule{2-8}
                               &                    Ours (Top1)                     &\textbf{   79.04  $\pm$ 0.48 {\color{olivegreen}(79.53)}}&\textbf{   70.59 $\pm$ 0.52 {\color{olivegreen}(71.04)}}&\textbf{   95.71  $\pm$ 0.06  {\color{olivegreen}(95.78)}}&\textbf{   92.50}$\pm$ 0.02 {\color{olivegreen}(92.52)} &\textbf{   69.44  $\pm$ 0.10 {\color{olivegreen}(69.53)}} &\textbf{   30.32 $\pm$ 0.07 {\color{olivegreen}(30.38)}} \\  
                               & Llama + ICL & 75.03 & 63.58 &  & & & \\
                               &                 Ours (Top3) + ICL                  &           76.93  $\pm$ 0.05 {\color{olivegreen}(76.98)} &           67.54 $\pm$ 0.04 {\color{olivegreen}(67.57)} &           95.43  $\pm$ 0.01  {\color{olivegreen}(95.44)} &           91.85 $\pm$ 0.01 {\color{olivegreen}(91.86)} &           65.81  $\pm$ 0.05 {\color{olivegreen}(65.86)}  &           27.86 $\pm$ 0.04 {\color{olivegreen}(27.89)}  \\  \midrule

            \multirow{8}{*}{16}&              BERT (Vanilla FT)                     &           75.52  $\pm$ 0.32 {\color{olivegreen}(76.07)} &           65.85 $\pm$ 1.28 {\color{olivegreen}(66.96)} &           95.31  $\pm$ 0.01  {\color{olivegreen}(95.37)} &           89.16 $\pm$ 0.07 {\color{olivegreen}(89.35)} &           70.97  $\pm$ 0.36 {\color{olivegreen}(71.32)}  &           30.90 $\pm$ 0.39 {\color{olivegreen}(31.34)}  \\
                               &  HiMatch \cite{chen-etal-2021-hierarchy}           &           77.67  $\pm$ 0.01 {\color{olivegreen}(78.24)} &           68.70 $\pm$ 0.01 {\color{olivegreen}(69.58)} &                                 -                        &                               -                        &                               -                          &                             -                           \\
                               &  HGCLR   \cite{wang-etal-2022-incorporating}       &           76.93  $\pm$ 0.52 {\color{olivegreen}(77.46)} &           67.92 $\pm$ 1.21 {\color{olivegreen}(68.66)} &           95.49  $\pm$ 0.04  {\color{olivegreen}(95.63)} &           89.41 $\pm$ 0.09 {\color{olivegreen}(89.71)} &           71.44  $\pm$ 0.38 {\color{olivegreen}(71.74)}  &           31.87 $\pm$ 0.05 {\color{olivegreen}(31.85)}  \\
                               &  HPT     \cite{wang-etal-2022-hpt}                 &           79.85  $\pm$ 0.41 {\color{olivegreen}(80.58)} &           72.02 $\pm$ 1.40 {\color{olivegreen}(73.31)} &           96.13  $\pm$ 0.01  {\color{olivegreen}(96.21)} &\underline{93.34}$\pm$ 0.02 {\color{olivegreen}(93.45)} &           73.23  $\pm$ 0.17 {\color{olivegreen}(73.37)}  &           33.44 $\pm$ 0.17 {\color{olivegreen}(33.60)}  \\
                               &  HierVerb \cite{ji-etal-2023-hierarchical} &\underline{80.93} $\pm$ 0.10 {\color{olivegreen}(81.26)} &\textbf{   73.80 $\pm$ 0.12 {\color{olivegreen}(74.19)}}&\underline{96.17} $\pm$ 0.01  {\color{olivegreen}(96.21)} &           93.28 $\pm$ 0.06 {\color{olivegreen}(93.49)} &\underline{75.72} $\pm$ 0.11 {\color{olivegreen}(75.85)}  &\underline{34.75}$\pm$ 0.10 {\color{olivegreen}(34.86)}  \\  \cmidrule{2-8}
                               &                    Ours (Top1)                     &\textbf{   81.12  $\pm$ 0.26 {\color{olivegreen}(81.38)}}&\underline{73.72}$\pm$ 0.17 {\color{olivegreen}(73.82)} &\textbf{   96.22  $\pm$ 0.04  {\color{olivegreen}(96.27)}}&\textbf{   93.37 $\pm$ 0.02 {\color{olivegreen}(93.46)}}&\textbf{   75.94  $\pm$ 0.11 {\color{olivegreen}(76.06)}} &\textbf{   34.95 $\pm$ 0.05 {\color{olivegreen}(35.00)}} \\
                               & Llama + ICL & 76.43 & 65.56 &  & & & \\
                               &                 Ours (Top3) + ICL                  &           78.62  $\pm$ 0.03 {\color{olivegreen}(78.65)} &           69.56 $\pm$ 0.03 {\color{olivegreen}(69.59)} &           95.56  $\pm$ 0.00  {\color{olivegreen}(95.56)} &           92.04 $\pm$ 0.00 {\color{olivegreen}(92.04)} &           68.73  $\pm$ 0.03 {\color{olivegreen}(68.76)}  &           29.82 $\pm$ 0.03 {\color{olivegreen}(29.85)}  \\
                               % \multicolumn{12}{c}{\textbf{Direct Model Transfer}} \\ \midrule
            % Src ${\dagger}$                 & 58.04 & 57.92 & 70.38 & 68.44 & 71.20 & 60.18 & 63.86 & 55.76 & 32.40 & 22.92 & 56.11 \\ 
            % Src ${\ddagger}$                & \textbf{69.60} & \textbf{67.31} & \textbf{78.36} & \textbf{75.43} & \textbf{77.58} & \textbf{66.10} & \textbf{68.81} & \textbf{65.18} & \textbf{43.26} & \textbf{32.05} & \textbf{64.37} \\ \midrule


            % \multicolumn{12}{c}{\textbf{Treebank Translation}} \\ \midrule
            % Tgt                             & 75.48 & 71.18 & 80.32 & 75.33 & 78.66 & 68.94 & 68.76 & 70.48 & 45.74 & 42.33 & 67.72 \\
            % Ours                            & \textbf{75.70} & \textbf{71.96} & \textbf{80.70} & \textbf{75.80} & \textbf{78.74} & \textbf{69.38} & \textbf{69.10} & \textbf{70.86} & \textbf{46.52} & \textbf{43.40} & \textbf{68.22} \\ \midrule
            % % Ours                            & 75.70 & 71.96 & 80.70 & 75.80 & 78.74 & 69.38 & 67.10 & 70.86 & 46.52 & 43.40 & 68.02 \\

            % Src+Tgt                         & 75.91 & 71.81 & 80.38 & 76.90 & 79.80 & 69.70 & 69.42 & 70.63 & 47.24 & 42.79 & 68.46 \\
            % Src+Ours                        & \textbf{76.48} & \textbf{72.68} & \textbf{80.74} & \textbf{76.99} & \textbf{80.14} & \textbf{69.80} & \textbf{70.30} & \textbf{71.22} & \textbf{47.98} & \textbf{43.73} & \textbf{69.01} \\ \bottomrule \toprule


            % \multicolumn{12}{c}{\textbf{Previous Works}} \\ \midrule

            % \newcite{ahmad2019cross}                     & 61.84 & 60.51 & 72.68 & 73.29 & 75.57 & 65.84 & 67.81 & 58.70 & 49.36 & 27.89 & 61.35 \\
            % % \newcite{zhang2019cross} ${\dagger}$         & 64.38 & -- & -- & 76.48 & 78.38 & 71.66 & 75.89 & -- & -- & -- & -- \\
            % \newcite{wang2019cross}                      & 64.78 & -- & 75.70 & 75.56 & 79.18 & 67.47 & 69.00 & 59.43 & -- & -- & -- \\
            % % \newcite{sun2020cross}                       & 63.39 & 64.09 & -- & 73.23 & 75.62 & 68.98 & -- & 61.87 & 53.77 & -- & -- \\
            % \newcite{kurniawan2021ppt}                   & 63.50 & 65.40 & 72.70 & 74.50 & 77.70 & 69.20 & \textbf{70.60} & -- & \textbf{53.90} & 38.50 & -- \\
            % \newcite{shi2021substructure}    & 71.70 & -- & -- & 71.00 & 75.00 & -- & -- & -- & -- & 41.30 & -- \\

        \bottomrule
    \end{tabular}
    }
    \caption{Micro-F1 and Macro-F1 scores on three datasets. We reported the average, standard deviation, and best results across three random seeds. \textbf{Bold}: best result. \underline{Underlined}: second highest.}
    \label{tab:main_result}
    \end{table*}


==> tables/main_result_cn_2col.tex <==
\begin{table}[t]
    \centering
    % \normalsize
    % \addtolength{\tabcolsep}{-3pt}
    \resizebox{1\columnwidth}{!}{
        \begin{tabular}{c l c c}
            \toprule
            
            \multirow{2}{*}{Q} & \makecell[c]{\multirow{2}{*}{Method}} & \multicolumn{2}{c}{\textbf{Patent(Depth 4)}} \\
            \cmidrule{3-4}
            & & Micro-F1 & Macro-F1 \\
            \midrule
            \multirow{9}{*}{1} & BERT (Vanilla FT) & 27.04  $\pm$ 1.48  {\color{olivegreen}(28.37)} & 2.40  $\pm$ 0.23 {\color{olivegreen}(2.67)} \\
                               & Llama-7B (Vanilla FT) & & \\
                               &  HiMatch \cite{chen-etal-2021-hierarchy}     & - & - \\
                               &  HGCLR \cite{wang-etal-2022-incorporating}       & 28.99  $\pm$ 1.12  {\color{olivegreen}(29.89)} &           2.94  $\pm$ 0.24 {\color{olivegreen}(3.13)}   \\
                               &  HPT     \cite{wang-etal-2022-hpt}                 & 35.22  $\pm$ 1.07  {\color{olivegreen}(36.26)} &           4.22  $\pm$ 0.68 {\color{olivegreen}(4.87)}   \\
                               &  HierVerb \cite{ji-etal-2023-hierarchical} &            41.83  $\pm$ 0.60  {\color{olivegreen}(42.52)} &           5.91  $\pm$ 0.65 {\color{olivegreen}(6.53)}   \\
                               \cmidrule{2-4}
                               &                    Ours Retrieval (Top1)                     & \underline{47.71} $\pm$ 0.41  {\color{olivegreen}(48.15)} &\underline{10.76}$\pm$ 0.25 {\color{olivegreen}(11.02)}  \\
                               & Ours Llama-7B (Top3) + ICL & & \\
                               &                 Ours ChatGPT (Top3) + ICL                  & \textbf{   52.23  $\pm$ 0.23  {\color{olivegreen}(52.45)}}&\textbf{   15.62 $\pm$ 0.17 {\color{olivegreen}(15.78)}} \\  \midrule

            \multirow{9}{*}{2} &              BERT (Vanilla FT)                     & 36.07  $\pm$ 0.24  {\color{olivegreen}(36.88)} &           6.41  $\pm$ 0.77 {\color{olivegreen}(6.92)}   \\
                               & Llama-7B (Vanilla FT) & & \\
                               &  HiMatch \cite{chen-etal-2021-hierarchy}           & - & - \\
                               &  HGCLR   \cite{wang-etal-2022-incorporating}       & 36.73  $\pm$ 1.13  {\color{olivegreen}(38.03)} &           6.82  $\pm$ 0.21 {\color{olivegreen}(7.06)}   \\
                               &  HPT     \cite{wang-etal-2022-hpt}                 & 42.61  $\pm$ 0.75  {\color{olivegreen}(43.43)} &           10.53 $\pm$ 0.30 {\color{olivegreen}(10.87)}  \\
                               &  HierVerb \cite{ji-etal-2023-hierarchical} &            48.42  $\pm$ 0.39  {\color{olivegreen}(48.74)} &           12.97 $\pm$ 0.39 {\color{olivegreen}(13.24)}  \\  \cmidrule{2-4}
                               &                    Ours (Top1)                     & \underline{51.63} $\pm$ 0.34  {\color{olivegreen}(51.91)} &\underline{15.12}$\pm$ 0.23 {\color{olivegreen}(15.32)}  \\  
                               & Llama + ICL & & \\
                               &                 Ours (Top3) + ICL                  & \textbf{   56.84  $\pm$ 0.11  {\color{olivegreen}(56.93)}}&\textbf{   20.07 $\pm$ 0.10 {\color{olivegreen}(20.17)}} \\  \midrule
            
            \multirow{8}{*}{4} &              BERT (Vanilla FT)                     & 9.64  $\pm$ 0.56 {\color{olivegreen}(10.13)} \\
                               &  HiMatch \cite{chen-etal-2021-hierarchy}           & -                        &                             -                          \\
                               &  HGCLR   \cite{wang-etal-2022-incorporating}       & 50.24 $\pm$ 0.36 {\color{olivegreen}(50.63)} &           11.40 $\pm$ 0.29 {\color{olivegreen}(11.67)} \\
                               &  HPT     \cite{wang-etal-2022-hpt}                 & 53.91 $\pm$ 0.44 {\color{olivegreen}(54.29)} &           18.45 $\pm$ 0.40 {\color{olivegreen}(18.79)} \\
                               &  HierVerb \cite{ji-etal-2023-hierarchical} &           72.58  $\pm$ 0.83 {\color{olivegreen}(73.64)} & 23.28 $\pm$ 0.39 {\color{olivegreen}(23.63)} \\
                               \cmidrule{2-4}
                               &                    Ours (Top1)                     & \textbf{   60.53 $\pm$ 0.36 {\color{olivegreen}(60.82)}}&\textbf{   25.65 $\pm$ 0.29 {\color{olivegreen}(25.95)}}\\  
                               & Llama + ICL & & \\
                               &                 Ours (Top3) + ICL                  & \underline{59.35}$\pm$ 0.10 {\color{olivegreen}(59.45)} &\underline{24.15}$\pm$ 0.08 {\color{olivegreen}(24.25)} \\  \midrule

            \multirow{8}{*}{8} &              BERT (Vanilla FT)                     & 26.85 $\pm$ 0.97 {\color{olivegreen}(27.75)}  \\
                               &  HiMatch \cite{chen-etal-2021-hierarchy}           & -                          &                             -                           \\
                               &  HGCLR   \cite{wang-etal-2022-incorporating}       & 64.69  $\pm$ 0.30 {\color{olivegreen}(65.01)}  &           27.69 $\pm$ 0.47 {\color{olivegreen}(28.21)}  \\
                               &  HPT     \cite{wang-etal-2022-hpt}                 & 67.35  $\pm$ 0.13 {\color{olivegreen}(67.45)}  &           28.39 $\pm$ 0.08 {\color{olivegreen}(28.46)}  \\
                               &  HierVerb \cite{ji-etal-2023-hierarchical} & \underline{68.74} $\pm$ 0.12 {\color{olivegreen}(68.82)}  &\underline{29.93}$\pm$ 0.07 {\color{olivegreen}(30.01)}  \\
                               \cmidrule{2-4}
                               &                    Ours (Top1)                     & \textbf{   69.44  $\pm$ 0.10 {\color{olivegreen}(69.53)}} &\textbf{   30.32 $\pm$ 0.07 {\color{olivegreen}(30.38)}} \\  
                               & Llama + ICL &  & \\
                               &                 Ours (Top3) + ICL                  & 65.81  $\pm$ 0.05 {\color{olivegreen}(65.86)}  &           27.86 $\pm$ 0.04 {\color{olivegreen}(27.89)}  \\  \midrule

            \multirow{8}{*}{16}&              BERT (Vanilla FT)                     & 30.90 $\pm$ 0.39 {\color{olivegreen}(31.34)}  \\
                               &  HiMatch \cite{chen-etal-2021-hierarchy}           & -                          &                             -                           \\
                               &  HGCLR   \cite{wang-etal-2022-incorporating}       & 71.44  $\pm$ 0.38 {\color{olivegreen}(71.74)}  &           31.87 $\pm$ 0.05 {\color{olivegreen}(31.85)}  \\
                               &  HPT     \cite{wang-etal-2022-hpt}                 & 73.23  $\pm$ 0.17 {\color{olivegreen}(73.37)}  &           33.44 $\pm$ 0.17 {\color{olivegreen}(33.60)}  \\
                               &  HierVerb \cite{ji-etal-2023-hierarchical} & \underline{75.72} $\pm$ 0.11 {\color{olivegreen}(75.85)}  &\underline{34.75}$\pm$ 0.10 {\color{olivegreen}(34.86)}  \\  \cmidrule{2-4}
                               &                    Ours (Top1)                     & \textbf{   75.94  $\pm$ 0.11 {\color{olivegreen}(76.06)}} &\textbf{   34.95 $\pm$ 0.05 {\color{olivegreen}(35.00)}} \\
                               & Llama + ICL & & \\
                               &                 Ours (Top3) + ICL                  & 68.73  $\pm$ 0.03 {\color{olivegreen}(68.76)}  &           29.82 $\pm$ 0.03 {\color{olivegreen}(29.85)}  \\
        \bottomrule
    \end{tabular}
    }
    \caption{Micro-F1 and Macro-F1 scores on three datasets. We reported the average, standard deviation, and best results across three random seeds. \textbf{Bold}: best result. \underline{Underlined}: second highest.}
    \label{tab:main_result}
    \end{table}

